Spectral asymptotics for Robin problems with a discontinuous coefficient

The spectral behavior of the difference between the resolvents of two realizations $\tilde A_1$ and $\tilde A_2$ of a second-order strongly elliptic symmetric differential operator $A$, defined by different Robin conditions $\nu u=b_1\gamma_0u$ and $\nu u=b_2\gamma_0u$, can in the case where all coefficients are $C^\infty$ be determined by use of a general result by the author in 1984 on singular Green operators. We here treat the problem for nonsmooth $b_i$. Using a Krein resolvent formula, we show that if $b_1$ and $b_2$ are in $L_\infty$, the s-numbers $s_j$ of $(\tilde A_1 -\lambda)^{-1}-(\tilde A_2 -\lambda)^{-1}$ satisfy $s_j j^{3/(n-1)}\le C$ for all $j$; this improves a recent result for $A=-\Delta $ by Behrndt et al., that $\sum_js_j ^p<\infty$ for $p>(n-1)/3$. A sharper estimate is obtained when $b_1$ and $b_2$ are in $C^\epsilon$ for some $\epsilon >0$, with jumps at a smooth hypersurface, namely that $s_j j^{3/(n-1)}\to c$ for $j\to \infty$, with a constant $c$ defined from the principal symbol of $A$ and $b_2-b_1$. As an auxiliary result we show that the usual principal spectral asymptotic estimate for pseudodifferential operators of negative order on a closed manifold extends to products of pseudodifferential operators interspersed with piecewise continuous functions.

==> gmacro1.tex <==
\def\slint{{\int\!\!\!\!\!\!@!@!@!@!{-}}}
\def\tslint{{\int\!\!\!\!\!@!@!@!{-}}}
\def\d{d\!@!@!@!@!@!{}^{@!@!\text{\rm--}}\!}
\def\dslash{d\!\!\!/ }
\def\fnorm{\|\!\!@!@!@!@!@!@!{}^{\text{\rm--}}}
\def\fscalar{(\!\!@!@!@!{}^{\text{\rm--}}}
\def\norm{{|@!@!@!@!|@!@!@!@!|}}
\def\wA{\widetilde A}
\def\wa{\tilde a}
\def\grad{\operatorname {grad}}
\def\divg{\operatorname {div}}
\def\supp{\operatorname{supp}}
\def\Cnul{C_0^{\infty}}
\def\C{C^{\infty}}
\def\Re{\operatorname{Re }}
\def\Im{\operatorname{Im }}
\def\pj{\operatorname {pr}_J}
\def\pjo{\operatorname{pr}_{J_0}}
\def\pjk{\operatorname{pr}_{J_k}}
\def\prk{\operatorname{pr}_k}
\def\pr{\operatorname{pr}}
\def\pb{{\operatorname{pr}}_{\beta }}%%virker ikke
\def\pg{{\operatorname{pr}}_{\gamma }}
\def\pg'{{\operatorname{pr}}_{\gamma '}}
\def\pz{{\operatorname{pr}}_{\zeta }}
\def\pb'{{\operatorname{pr}}_{\beta '}}
\def\pz'{{\operatorname{pr}}_{\zeta '}}
\def\Hloc#1{H^{\operatorname{loc}}_{(#1)}} 
\def\vn{{\vec n}}
\def\new{\qquad {\tt new text}\qquad }
\def\old#1#2{\flushpar{\tt Page #1, line #2: old text}\qquad }
\def\Hnul#1#2{H_{(0)}^{#1}(#2)} 
\def\H#1#2{H^{#1}(#2)} 
\def\nye{\qquad {\tt ny tekst}\qquad }
\def\gamle#1#2{\flushpar{\tt Side #1, linie #2: gammel tekst}\qquad }
\def\tilf#1#2{\flushpar{\tt Side #1, linie #2, tilf\o{}j:}\qquad }
\def\add#1#2{\flushpar{\tt Side #1, linie #2, add:}\qquad }
\def\replace#1#2{\flushpar{\tt Page #1, line #2, replace:}\qquad }
\def\byy{\qquad {\tt by:}\qquad }
\def\change#1#2{\flushpar{\tt Page #1, line #2, change:}\qquad }
\def\too{\qquad {\tt to:}\qquad }
\def\erstat#1#2{\flushpar{\tt Side #1, linie #2, erstat:}\qquad }
\def\med{\qquad {\tt med:}\qquad }
\def\pr{\operatorname{pr}}
\def\leg{\;\dot{\le}\;}
\def\geg{\;\dot{\ge}\;}
\def\eg{\;\dot {=}\;}
\def\crp{\overline{\Bbb R}_+}
\def\crm{\overline{\Bbb R}_-}
\def\crpm{\overline{\Bbb R}_\pm}
\def\rn{{\Bbb R}^n}
\def\rnp{{\Bbb R}^n_+}
\def\rnm{\Bbb R^n_-}
\def\rnpm{\Bbb R^n_\pm}
\def\crnp{\overline{\Bbb R}^n_+}
\def\crnm{\overline{\Bbb R}^n_-}
\def\crnpm{\overline{\Bbb R}^n_\pm}
\def\comega{\overline\Omega }
\def\srplus{\Cal S(\overline{\Bbb R}_+)}
\def\srminus{\Cal S(\overline{\Bbb R}_-)}
\def\srnp{\Cal S(\overline{\Bbb R}^n_+)}
\def\srnpm{\Cal S(\overline{\Bbb R}^n_\pm)}
\def\ch{\Cal H}
\def\chp{\Cal H^+}
\def\chm{\Cal H^-}
\def\chpm{\Cal H^\pm}
\def\Rn{\Bbb R^n}
\def\ang#1{\langle {#1} \rangle}
\def\lag{\Bbb R^{n-1}\times\Bbb R}
\def\H{\overline H}
\def\Op{\operatorname{Op}}
\def\Pfrac{\tsize\frac1{\raise 1pt\hbox{$\scriptstyle p$}}}
\def\pfrac{\frac1{\raise 1pt\hbox{$\scriptscriptstyle p$}}}
\def\Pfracc#1{\tsize\frac{#1}{\raise 1pt\hbox{$\scriptstyle p$}}}
\def\pfracc#1{\frac{#1}{\raise 1pt\hbox{$\scriptscriptstyle p$}}}
\def\rnprod{\Bbb R^{n-1}\!\times\!\overline{\Bbb R}^n_+}
\def\inv{^{-1}}
\def\simto{\overset\sim\to\rightarrow}
\def\ttilde{\overset{\,\approx}\to}
\def\set#1{\{{#1}\}}
\def\Cnoll{\Cnul}
\def\scalar#1#2{\langle#1,#2\rangle}
\def\domain#1{\{\,#1\,\}}
\def \im{\text{\rm i}}
\def\Zfrac{\tsize\frac1{\raise 1pt\hbox{$\scriptstyle z$}}}
\def\zfrac{\frac1{\raise 1pt\hbox{$\scriptscriptstyle z$}}}
%\def\d{d\!\!\!/ }
\def\crpp{\overline {\Bbb R}^2_{++}}
\def\rpp{ {\Bbb R}^2_{++}}
\def\rp{ \Bbb R_+}
\def\rmi{ \Bbb R_-}
\define\tr{\operatorname{tr}}
\define\op{\operatorname{OP}}
\define\Tr{\operatorname{Tr}}
\define\TR{\operatorname{TR}}
\define\srplusp{\Cal S(\crpp)}
\define\srp{\Cal S_+}
\define\srm{\Cal S_-}
\define\srpm{\Cal S_\pm}
\define\srpp{\Cal S_{++}}
\define\stimes{\!\times\!}

\def\ur{\underline r}
\define\up{\underline p}
\define\uq{\underline q}
\define\uP{\underline P}
\define\ux{\underline x}
\define\uy{\underline y}
\define\uu{\underline u}
\define\uv{\underline v}
\define\uxi{\underline \xi}
\define\ueta{\underline \eta}
\define\uG{\underline G}
\define\uT{\underline T}
\define\uH{\underline H}
\define\uE{\underline E}
\define\uF{\underline F}
\define\uK{\underline K}
\define\ug{\underline g}
\define\ut{\underline t}
\define\uk{\underline k}
\define\uomega{\underline \Omega}

